On Treewidth and Stable Marriage

Stable Marriage is a fundamental problem to both computer science and economics. Four well-known NP-hard optimization versions of this problem are the Sex-Equal Stable Marriage (SESM), Balanced Stable Marriage (BSM), max-Stable Marriage with Ties (max-SMT) and min-Stable Marriage with Ties (min-SMT) problems. In this paper, we analyze these problems from the viewpoint of Parameterized Complexity. We conduct the first study of these problems with respect to the parameter treewidth. First, we study the treewidth $\mathtt{tw}$ of the primal graph. We establish that all four problems are W[1]-hard. In particular, while it is easy to show that all four problems admit algorithms that run in time $n^{O(\mathtt{tw})}$, we prove that all of these algorithms are likely to be essentially optimal. Next, we study the treewidth $\mathtt{tw}$ of the rotation digraph. In this context, the max-SMT and min-SMT are not defined. For both SESM and BSM, we design (non-trivial) algorithms that run in time $2^{\mathtt{tw}}n^{O(1)}$. Then, for both SESM and BSM, we also prove that unless SETH is false, algorithms that run in time $(2-\epsilon)^{\mathtt{tw}}n^{O(1)}$ do not exist for any fixed $\epsilon>0$. We thus present a comprehensive, complete picture of the behavior of central optimization versions of Stable Marriage with respect to treewidth.

==> preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}
\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{todonotes}

\newcommand{\OO}{\mathcal{O}}

\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{redrule}{Reduction Rule}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{reduction}{Reduction Rule}[section]
\newtheorem{conjecture}{Conjecture}[section]

\date{}
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

\newcommand{\sesm}{{\sc SESM}}
\newcommand{\alg}{{\sc ALG-GSM}}
\newcommand{\var}{\mbox{\sf var}}
\newcommand{\posi}{\mbox{\sf pos}}
\newcommand{\nega}{\mbox{\sf neg}}
\newcommand{\nil}{\mbox{\sf nil}}
\newcommand{\partner}{\mbox{\sf par}}
\newcommand{\cl}{\mbox{\sf cl}}
\newcommand{\rootT}{\mbox{\sf root}}
\newcommand{\pos}{\mbox{\sf p}}
\newcommand{\sat}{\mbox{\sf sat}}
\newcommand{\diff}{\mbox{\sf diff}}
\newcommand{\rep}{\mbox{\sf rep}}
\newcommand{\domain}{\mbox{\sf dom}}
\newcommand{\image}{\mbox{\sf ima}}
\newcommand{\bal}{\ensuremath{{\sf bal}}}
\newcommand{\Bal}{\ensuremath{{\sf Bal}}}
\newcommand{\bas}{\mbox{\sf bas}}
\newcommand{\enr}{\mbox{\sf enr}}
\newcommand{\hap}{\mbox{\sf hap}}
\newcommand{\red}{\mbox{\sf red}}

\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
\newcommand{\algSESM}{{\ttfamily{SESM-ALG}}}
\newcommand{\algBSM}{{\ttfamily{BSM-ALG}}}
\newcommand{\algSAT}{{\ttfamily{SAT-ALG}}}
\newcommand{\tw}{\mathtt{tw}}
\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\XP}{\text{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref} 


